Graph Edits for Counterfactual Explanations: A comparative study

Counterfactuals have been established as a popular explainability technique which leverages a set of minimal edits to alter the prediction of a classifier. When considering conceptual counterfactuals on images, the edits requested should correspond to salient concepts present in the input data. At the same time, conceptual distances are defined by knowledge graphs, ensuring the optimality of conceptual edits. In this work, we extend previous endeavors on graph edits as counterfactual explanations by conducting a comparative study which encompasses both supervised and unsupervised Graph Neural Network (GNN) approaches. To this end, we pose the following significant research question: should we represent input data as graphs, which is the optimal GNN approach in terms of performance and time efficiency to generate minimal and meaningful counterfactual explanations for black-box image classifiers?

==> combined_metrics.tex <==
\begin{table}
\small
    \centering
    \caption{Combined Counterfactual retrieval results with Supervised and Unsupervised GNN architectures. \underline{Underlined} cells indicate best results per graph model (kernel, supervised, unsupervised). \textbf{Bold} denotes best results overall per dataset split.}
    \label{tab:combined-gnn-results}
    \vskip 0.1in
    \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \toprule
    & \multicolumn{6}{c}{\small NDCG} & \multicolumn{6}{c}{\small Precision (P)} \\ 
    \cline{2-13}
Model & @4	& @2 & @1  & @4 & @2 & @1 & @4	& @2 & @1  & @4 & @2 & @1 \\
\midrule
    \multicolumn{13}{c}{\small VG-DENSE} \\
    \midrule
WL kernel & \underline{0.219} & \underline{0.219} & \underline{0.224} & \underline{0.164} & 0.125 & 0.076 & 0.186 & 0.128 & 0.076 & 0.164 & 0.128 & 0.076 \\
SP kernel & 0.201 & 0.205 & 0.205& 0.154 & \underline{0.145} & \underline{0.122} & \underline{0.232} & \underline{0.174} & \underline{0.122} & \underline{0.232} & \underline{0.174} & \underline{0.122} \\
RW kernel & 0.002 & 0.002 & 0.0& 0.001 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
NH kernel & 0.115 & 0.116 & 0.107 & 0.088 & 0.073 & 0.05 & 0.124 & 0.086 & 0.05 & 0.124 & 0.086 & 0.05 \\
GS kernel & 0.029 & 0.026 & 0.026 & 0.022 & 0.007 & 0.008 & 0.018 & 0.008 & 0.008 & 0.002 & 0.0 & 0.0 \\
\midrule
Superv. GAT & 0.400 & 0.39 & 0.375 & 0.312 & 0.25 & 0.164 & 0.422 & 0.288 & 0.164 & 0.492 & 0.37 & 0.248 \\
Superv. GIN & 0.346 & 0.346 & 0.338 & 0.252 & 0.192 & 0.158 & 0.344 & 0.242 & 0.158 & 0.344 & 0.242 & 0.158\\
Superv. GCN & \textbf{0.457} & \textbf{0.456} & \textbf{}\textbf{0.445} & \textbf{0.358} & \textbf{0.292} & \textbf{0.248} & \textbf{0.492} & \textbf{0.37} & \textbf{0.248} & \textbf{0.492} & \textbf{0.37} & \textbf{0.248} \\
\midrule
GAE GAT & 0.103 & 0.11 & 0.109 & 0.075 & 0.075 & 0.048 & 0.108 & 0.078 & 0.048 & 0.108 & 0.078 & 0.048 \\
GAE GIN & 0.116 & 0.121 & 0.119 & 0.082 & 0.078 & 0.052 & 0.132 & 0.098 & 0.052 & 0.132 & 0.098 & 0.052 \\
GAE GCN & 0.091 & 0.096 & 0.094 & 0.071 & 0.06 & 0.052 & 0.102 & 0.078 & 0.052 & 0.102 & 0.078 & 0.052 \\
VGAE GAT & 0.189 & 0.193 & 0.185& 0.139 & 0.12 & 0.082 & 0.196 & 0.138 & 0.082 & 0.196 & 0.138 & 0.082 \\
VGAE GIN & 0.190 & 0.194 & 0.192 & \underline{0.141} & 0.119 & 0.09 & 0.202 & 0.146 & 0.09 & 0.202 & 0.146 & 0.09 \\
VGAE GCN & 0.167 & 0.169 & 0.161 & 0.122 & 0.101 & 0.066 & 0.174 & 0.118 & 0.066 & 0.174 & 0.118 & 0.066 \\
GFA GAT & 0.178 & 0.184 & 0.178 & 0.122 & 0.109 & 0.086 & 0.182 & 0.14 & 0.086 & 0.182 & 0.14 & 0.086 \\
GFA GIN & 0.191 & 0.195 & 0.195 & 0.14 & 0.122 & 0.096 & 0.21 & 0.148 & 0.096 & 0.21 & 0.148 & 0.096 \\
GFA GCN & 0.163 & 0.165 & 0.158 & 0.12 & 0.104 & 0.068 & \underline{0.289} &\underline{0.2} & \underline{0.139} & \underline{0.289} &\underline{0.2} & \underline{0.139} \\
ARVGA GAT & 0.181 & 0.186 & 0.18 & 0.132 & 0.114 & 0.084 & 0.188 & 0.14 & 0.084 & 0.188 & 0.14 & 0.084 \\
ARVGA GIN & \underline{0.192} & \underline{0.2} & \underline{0.199} & 0.135 & \underline{0.124} & \underline{0.106} & 0.218 & 0.164 & 0.106 & 0.218 & 0.164 & 0.106 \\
ARVGA GCN & 0.170 & 0.174 & 0.17 & 0.122 & 0.106 & 0.076 & 0.184 & 0.138 & 0.076 & 0.184 & 0.138 & 0.076 \\
\midrule
    \multicolumn{13}{c}{\small VG-RANDOM} \\
    \midrule
WL kernel & 0.189 & 0.192 & \underline{0.213} & 0.13 & \underline{0.108} & \underline{0.096} & 0.166 & \underline{0.124} & \underline{0.096} & 0.166 & \underline{0.124} & \underline{0.096} \\
SP kernel & 0.115 & 0.118 & 0.123& 0.079 & 0.068 & 0.064 & 0.11 & 0.09 & 0.064 & 0.11 & 0.09 & 0.064 \\
RW kernel & 0.012 & 0.01 & 0.009 & 0.007 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
NH kernel & \underline{0.19} & \underline{0.196} & 0.212 & \underline{0.135} & 0.116 & 0.092 & \underline{0.168} & 0.116 & 0.092 & \underline{0.168} & 0.116 & 0.092 \\
GS kernel & 0.007 & 0.006 & 0.003 & 0.05 & 0.0 & 0.0 & 0.002 & 0.0 & 0.0 & 0.002 & 0.0 & 0.0 \\
\midrule
Superv. GAT & 0.394 & 0.396 & 0.395 & 0.294 & 0.245 & 0.176 & 0.382 & 0.294 & 0.176 & 0.382 & 0.294 & 0.176 \\
Superv. GIN & 0.333 & 0.337 & 0.34 & 0.245 & 0.205 & 0.144 & 0.308 & 0.228 & 0.144 & 0.308 & 0.228 & 0.144 \\
Superv. GCN & \textbf{0.400} & \textbf{0.397} & \textbf{0.401} & \textbf{0.295} & \textbf{0.246} & \textbf{0.2} & \textbf{0.424} & \textbf{0.3} & \textbf{0.2} & \textbf{0.424} & \textbf{0.3} & \textbf{0.2} \\
\midrule
GAE GAT & 0.132 & 0.14 & 0.151 & 0.092 & 0.085 & 0.07 & 0.132 & 0.104 & 0.07 & 0.132 & 0.104 & 0.07 \\
GAE GIN & 0.117 & 0.127 & 0.133 & 0.08 & 0.076 & 0.07 & 0.114 & 0.096 & 0.07 & 0.114 & 0.096 & 0.07 \\
GAE GCN & 0.12 & 0.13 & 0.141 & 0.079 & 0.078 & 0.066 & 0.114 & 0.1 & 0.066 & 0.114 & 0.1 & 0.066 \\
VGAE GAT & 0.158 & 0.17 & 0.182 & 0.103 & 0.1 & 0.09 & 0.16 & 0.122 & 0.09 & 0.16 & 0.122 & 0.09 \\
VGAE GIN & 0.16 & 0.173 & 0.186 & 0.11 & 0.101 & 0.088 & 0.152 & 0.118 & 0.088 & 0.152 & 0.118 & 0.088 \\
VGAE GCN & 0.156 & 0.167 & 0.18 & 0.101 & 0.089 & 0.088 & \underline{0.156} & 0.122 & 0.088 & \underline{0.156} & 0.122 & 0.088 \\
GFA GAT & 0.157 & 0.169 & 0.185 & 0.107  & 0.094 & 0.076 & 0.142 & 0.108 & 0.076 & 0.142 & 0.108 & 0.076 \\
GFA GIN & 0.158 & 0.17 & 0.183 & 0.11 & 0.093 & 0.082 & 0.142 & 0.11 & 0.082 & 0.142 & 0.11 & 0.082 \\
GFA GCN & 0.157 & 0.168 & 0.184 & 0.106 & 0.095 & 0.082 & 0.14 & 0.112 & 0.082 & 0.14 & 0.112 & 0.082 \\
ARVGA GAT & 0.167 & 0.18 & 0.193 & 0.111 & \underline{0.103} & 0.092 & \underline{0.156} & \underline{0.13} & 0.092 & \underline{0.156} & \underline{0.13} & 0.092 \\
ARVGA GIN & \underline{0.17} & \underline{0.181} & \underline{0.194} & \underline{0.116} & 0.099 & 0.084 & 0.152 & 0.118 & 0.084 & 0.152 & 0.118 & 0.084\\
ARVGA GCN & 0.166 & 0.179 & 0.193 & 0.113 & 0.097 & \underline{0.094} & 0.154 & \underline{0.13} & \underline{0.094} & 0.154 & \underline{0.13} & \underline{0.094} \\
    \bottomrule
    \end{tabular}

\end{table}


==> combined_table.tex <==
\begin{table}[h!]
\centering
\caption{Average Number of Edits in terms of nodes, edges and total, as well as Top-1 GED Values for counterfactual instances retrieved for VG-DENSE and VG-RANDOM.}
\label{tab:combined_metrics}
\vskip 0.1in
\begin{tabular}{l|ccc|c}
\toprule
Model & Node $\downarrow$ & Edge $\downarrow$ & Total $\downarrow$ & GED $\downarrow$ \\
\midrule
\multicolumn{5}{c}{\small VG-DENSE} \\
\midrule
WL kernel & 5.24 & 11.668 & 16.908 & 130.146 \\
SP kernel & \underline{4.964} & 12.078 & 17.042 & \underline{129.334} \\
RW kernel & 9.162 & 20.006 & 29.168 & 217.684 \\
NH kernel & 5.348 & \underline{11.264} & 16.612 & 141.18 \\
GS kernel & 6.444 & 16.748 & 23.192 & 178.434 \\
\midrule
Superv. GAT & 5.278 & 10.892 & 16.17 & 108.636 \\
Superv. GIN & 5.106 & 10.766 & 15.872 & 116.174 \\
Superv. GCN & \underline{4.942} & \textbf{10.312} & \textbf{15.254} & \textbf{105.194} \\
\midrule
GAE GAT & 5.504 & 11.848 & 17.352 & 143.976 \\
GAE GIN & 5.4 & 12.002 & 17.402 & 143.182 \\
GAE GCN & 5.178 & 11.27 & 16.448 & 143.506 \\
VGAE GAT & 5.03 & 11.4 & 16.43 & 130.124 \\
VGAE GIN & 4.918 & 10.97 & 15.888 & 131.514 \\
VGAE GCN & 5.114 & 11.702 & 16.816 & 132.056 \\
GFA GAT & 5.07 & 11.564 & 16.634 & 131.582 \\
GFA GIN & \textbf{4.856} & \underline{10.786} & 15.642 & 129.856 \\
GFA GCN & 5.03 & 11.432 & 16.462 & 132.046 \\
ARVGA GAT & 5.062 & 11.482 & 16.544 & 133.476 \\
ARVGA GCN & 5.048 & 11.316 & 16.364 & 132.294 \\
ARVGA GIN & 4.894 & 10.912 & 15.806 & \underline{128.944} \\
\midrule
\multicolumn{5}{c}{\small VG-RANDOM} \\
\midrule
WL kernel & 13.44 & 11.946 & 25.386 & 192.824 \\
SP kernel & 14.144 & 12.386 & 26.53 & 208.096 \\
RW kernel & 17.814 & 22.36 & 40.174 & 385.726 \\
NH kernel & \underline{12.568} & \underline{11.714} & \underline{24.282} & \underline{190.376} \\
GS kernel & 17.216 & 15.344 & 32.56 & 272.744 \\
\midrule
Superv. GAT & 12.81 & 11.978 & 24.788 & \textbf{159.324} \\
Superv. GIN & 12.792 & \underline{11.394} & \underline{24.186} & 173.72 \\
Superv. GCN & \underline{12.392} & 11.84 & 24.232 & 159.356 \\
\midrule
GAE GAT & \textbf{11.952} & 11.426 & \textbf{23.378} & 197.626 \\
GAE GIN & 12.554 & 11.738 & 24.292 & 201.638 \\
GAE GCN & 12.134 & \textbf{11.384} & 23.518 & 202.638 \\
VGAE GAT & 12.884 & 12.376 & 25.26 & 197.226 \\
VGAE GIN & 12.692 & 12.042 & 24.734 & 199.34 \\
VGAE GCN & 12.91 & 12.392 & 25.302 & \underline{195.938} \\
GFA GAT & 12.988 & 12.412 & 25.4 & 198.78 \\
GFA GIN & 12.916 & 12.218 & 25.134 & 200.974 \\
GFA GCN & 12.696 & 12.338 & 25.034 & 201.038 \\
ARVGA GAT & 12.508 & 12.192 & 24.7 & 196.946 \\
ARVGA GIN & 12.234 & 11.794 & 24.028 & 198.654 \\
ARVGA GCN & 12.464 & 12.088 & 24.552 & 198.46 \\
\bottomrule
\end{tabular}
\end{table}
